Mobile Internet Experience: Urban vs. Rural -- Saturation vs. Starving?

Mobile Internet experience has been of increasing interest. Services accessed via smartphone applications shall provide satisfying Quality of Experience (QoE), irrespective of end user location, time of the day, and other circumstances. Unfortunately, current LTE networks often don't provide constant user throughput, one of the major system influence factors to mobile Internet QoE. In this paper, we conducted an exemplary measurement study in LTE networks, comparing the QoE of mobile networks in an urban and a rural region. Our results show that there are significant differences concerning the network speed which can result in unsatisfactory service quality depending on the application to be used. When evaluating the QoE for multiple users who are using the same base station in a specific area, user satisfaction decreases drastically, especially in rural areas. Our work encourages for future work to focus on this gap between the QoE in urban and rural areas.

==> sections/relatedWork.tex <==
\section{Background and Related Work}\label{sec:related-work}

\todo{}







